Incentivizing Vision Language Models to Search for Long Video Question Answering

We introduce VSeek, an agentic framework that transforms long-video question answering (LVQA) from a passive, single-pass perception task into a multi-turn retrieval process. VSeek utilizes a natural language-driven search to identify relevant context within long videos and is post-trained with reinforcement learning (RL) to jointly formulate targeted search queries and reason over retrieved clips for LVQA. While RL post-training has revolutionized reasoning in symbolic domains such as mathematics and code, its application to long-video understanding remains hindered by a lack of verified rewards. To ensure that the retrieved context is relevant, we propose a novel neuro-symbolic approach that bridges open-ended natural language with discrete visual verification. Specifically, complex user queries are compiled into formal temporal logic specifications for systematically decomposing natural language questions into a definitive checklist of required atomic visual primitives, such as key objects and activities, along with their temporal ordering. These systematically derived grounding events provide the critical feedback signal for RL post-training, enabling dense, verifiable rewards based on the successful retrieval of these specific visual elements rather than relying entirely on outcome-only answer accuracy. By explicitly optimizing for this verifiable evidence-seeking behavior, VSeek improves Pass@1 scores by up to 8% and Pass@4 scores by 15% on long-video understanding benchmarks compared to base models. We open-source our code at https://utaustin-swarmlab.github.io/VSeek.

==> tex/intro_old.tex <==
\section{Introduction}


The exponential growth of long-form video content—ranging from surveillance footage and movies to instructional tutorials—presents a fundamental challenge for computer vision: accurately comprehending and reasoning over extended temporal contexts. While recent advancements in Large Vision-Language Models (VLMs) have expanded context windows to handle millions of tokens [17, 25], raw capacity does not equate to reasoning capability. When faced with hour-long videos, simply feeding the entire sequence into a model often leads to information overload, where the model struggles to distinguish fine-grained details from irrelevant background noise.

To address this, the field has increasingly pivoted toward Retrieval-Augmented Generation (RAG) and neuro-symbolic approaches. Frameworks like Neus-QA attempt to bridge this gap by relying on external modules to pre-select frames or generate symbolic representations before the VLM processes the query. However, these methods effectively decouple the searching process from the reasoning process. The retrieval mechanism is often static or rule-based, unable to dynamically adapt its search strategy based on partial evidence found during the inference process. We posit that to truly solve long-video Question Answering (QA), a model must possess "active vision"—the ability to intrinsically interleave tool use with temporal reasoning, iteratively searching the video environment to construct its own context.

In this work, we introduce VSeek, an agentic framework designed to transform long-video QA from a passive perception task into an active, multi-turn discovery process. Unlike standard single-turn RAG methods that retrieve context once based on the initial query, VSeek operates as an autonomous agent. It decomposes complex user queries, formulates targeted search strings to retrieve specific video segments, and refines its understanding iteratively. However, the realization of such an agentic framework is non-trivial. Through a rigorous empirical investigation, we identify and address the critical failure modes that plague autonomous video agents. Our initial evaluations revealed that naive implementations of VLM agents often perform worse than random guessing, not due to a lack of visual perception, but due to deficiencies in reasoning and context management. We demonstrate that simply enabling tool use is insufficient; the structure of the retrieved information is paramount. We show that temporal alignment—reordering retrieved clips to match their original sequence—is a strict requirement for preserving causal reasoning, without which the agent hallucinates temporal relationships.

Furthermore, we uncover a significant "reasoning bottleneck" in standard base models (e.g., Qwen2.5-VL). Our experiments with sparse-frame overviews indicate that providing more visual context fails if the underlying model lacks the planning capability to utilize it. We show that transitioning to "Thinking" models (e.g., Qwen 3) significantly alleviates this, validating the hypothesis that agentic video understanding is bound by the model’s ability to maintain a coherent Chain of Thought (CoT).Finally, we address the instability of training these agents via Reinforcement Learning (RL).

A recurring challenge in training VLM agents is "formatting brittleness" and premature convergence. We present an analysis of policy entropy during RL training, demonstrating that a rapid collapse in entropy leads to deterministic, suboptimal policies. We propose and validate a learning rate warmup schedule that regulates entropy decay, ensuring sufficient exploration of the tool-use space and preventing performance collapse.Our contributions are summarized as follows:We propose VSeek, an agentic framework that outperforms single-turn RAG by allowing VLMs to reason and search a video repeatedly, effectively locating contextual information in long-form content.

We provide a systematic analysis of retrieval dynamics, establishing that temporal reordering and an optimized top-$k$ retrieval strategy (peaking at $k=4$ with 8-second clips) are essential for maximizing agent accuracy.We identify the "entropy collapse" phenomenon in RL fine-tuning for video agents and demonstrate that controlled entropy decay via learning rate warmup is critical for learning robust, high-performing policies.We demonstrate that the primary bottleneck for agentic video QA is the reasoning capacity of the base model, showing that "Thinking" models capable of internal monologue significantly outperform standard instruction-tuned models in multi-step visual search tasks.

==> tex/preamble.tex <==
\usepackage{esvect}
\newcommand{\harsh}[1]{\textcolor{red}{Harsh: #1}}

\DeclareMathOperator*{\argmax}{arg\,max}



\newcommand{\trajt}[1]{\tau^i_{#1}}

\newcommand{\typet}[2]{\psi^{#2}_{#1}}
\newcommand{\jointtypet}[2]{\boldsymbol{\psi}^{#2}_{#1}}

\newcommand{\obst}[1]{o^i_{#1}}

\newcommand{\actego}[1]{a^i_{#1}}
\newcommand{\policyego}[1]{\pi^i_{#1}}
\newcommand{\actteam}[2]{a^{#2}_{#1}}
\newcommand{\policyteam}[2]{\pi^{#2}_{#1}}

\newcommand{\typeinitdist}{\rho_{0}^{\tau}}
\newcommand{\stateinitdist}{\rho_{0}^{s}}

\newcommand{\historyem}{\theta_{e}}
\newcommand{\roleenc}{\theta_{r}}
\newcommand{\globalq}{Q_{tot}^{\pi}}


\newcommand{\gain}[2]{\shortstack{#1\\[-0.3ex]{\scriptsize\textcolor{green!60!black}{#2}}}}
\newcommand{\drop}[2]{\shortstack{#1\\[-0.3ex]{\scriptsize\textcolor{red!70!black}{#2}}}}
